FPCD: An Open Aerial VHR Dataset for Farm Pond Change Detection

Change detection for aerial imagery involves locating and identifying changes associated with the areas of interest between co-registered bi-temporal or multi-temporal images of a geographical location. Farm ponds are man-made structures belonging to the category of minor irrigation structures used to collect surface run-off water for future irrigation purposes. Detection of farm ponds from aerial imagery and their evolution over time helps in land surveying to analyze the agricultural shifts, policy implementation, seasonal effects and climate changes. In this paper, we introduce a publicly available object detection and instance segmentation (OD/IS) dataset for localizing farm ponds from aerial imagery. We also collected and annotated the bi-temporal data over a time-span of 14 years across 17 villages, resulting in a binary change detection dataset called \textbf{F}arm \textbf{P}ond \textbf{C}hange \textbf{D}etection Dataset (\textbf{FPCD}). We have benchmarked and analyzed the performance of various object detection and instance segmentation methods on our OD/IS dataset and the change detection methods over the FPCD dataset. The datasets are publicly accessible at this page: \textit{\url{https://huggingface.co/datasets/ctundia/FPCD}}

==> augmentation.tex <==

\subsection{Change and Instance Augmentation}
\label{subsection:Change and Instance augmentation}
\noindent
To deal with the above issues, we propose Instance and Change mask augmentation, which are motivated by the copy-paste augmentation \cite{copy_paste_2021_CVPR}. 
%We introduce two augmentation techniques for multi-class change detection task with subtleties in their implementation. 
The augmentations can be classified into two: instance augmentation and change mask augmentation, based on whether the generated mask label is different from the original change mask label. The implementation of both augmentations vary when applied to positive and negative change object images.
\par
Instance augmentation preserves the original label by replacing an existing object by an instance of another object of the same category. As the result, the change label doesn't alter after instance augmentation. For each object annotation in an input image, a candidate instance is found, which generally belongs to the same category. Once a candidate instance is identified, the annotation for the same is loaded and the instance is cropped out from its' image. To keep the location and dimensions of the label mask constant, the new object is resized to the same dimensions of the original object annotation and placed at the same location. A change is categorized and assigned a change color based on the change in category between the source and target objects at the same position. Change augmentation doesn't preserve the original label by replacing an existing object annotation by any instance of another category. For MIS-FPCD dataset, we apply instance and change-mask annotations differently for positive instance images and no-instance images. 

With instance augmentation there are two different ways that can generate different results. For each candidate annotation that will replace the existing annotation, if we use the same position of the existing annotation the change mask will remain the same. However, this can lead to the model overfitting the mask labels. To avoid this issue, we take the position of the new annotation and place the object instance in a new position. As a result, new mask labels belong mostly to red and green color for change classes farmpond demolished and farmpond constructed, respectively. We use this variant, named as as $Instance_{new}^{pos}$ augmentation, whenever we use Instance augmentation for augmenting positive images. Refer Figure \ref{fig:pos2pos_instance} for the illustration.

With change mask augmentation, there are two different ways that can result in different outcomes, based on the position to place the new annotations. On keeping the positions from the new annotations, the new mask labels belong mostly to red and green color for change classes farmpond demolished and farmpond constructed, respectively. However, on keeping the original position, this generates both yellow and blue change masks, farmpond dried and farmpond wetted, respectively. We use this variant, named as $Change mask_{old}^{pos}$ augmentation, whenever we use Change mask augmentation for augmenting positive images. Refer Figure \ref{fig:pos2pos_change} for the illustration.

Similarly, for augmenting bi-temporal negative image pair, there are two different ways that can generate different results. Refer Figure \ref{fig:negtopos} for negative to positive augmentation. Either, we can place the annotations in random locations on the negative images or we can take the location information from ground truth object instances from positive images. Using existing annotations from positive images and placing them on the negative images helps to treat negative images as positive image, enabling the same set of above augmentations to be applied.

The negative-image pair can borrow different set of annotations from two different positive images or duplicate the same set of annotations from a single positive image. In the former case, both instance and change mask annotations generate the new mask labels belonging to red and green color for change classes, farmpond demolished and farmpond constructed, respectively. In the latter case, instance augmentation by keeping the old annotation's position generates yellow and blue masks while instance augmentation by keeping the new annotation's position leads to red and green masks. We use the second variant, named as $Instance_{new}^{neg}$ augmentation, whenever we use Instance mask augmentation for augmenting negative images. 

Similarly, change mask augmentation generates two results based on whether to use the new position or old position. Using the new position leads to red and green masks, while using the old position leads to yellow and blue masks. We use the second variant, named as $Change mask_{old}^{neg}$ augmentation, whenever we use Change mask augmentation for augmenting negative images.

The results in the Table \ref{tab:results_augmentations} suggest that only change mask augmentations and both instance and change mask augmentations improved the f-score. As discussed before, $Instance_{new}^{neg}$ augmentation results in red and green masks, of which green label mask are already over-represented in the original dataset. While red label mask instances are increased by augmentation, it is easy for the model to detect the green and red mask, since only one of the inputs have the object at that co-registered point. 
However, yellow and blue masks involve correctly identifying the category of both the input objects before predicting the change mask. Since, $Instance_{new}^{neg}$ augmentation generates new red and green masks, and $Change_{old}^{neg}$ generates both yellow and blue masks,  the model benefits from the $Change_{old}^{neg}$ augmentation. In short, when there are farmponds created or destroyed the model can easily identify the change as green or red but it is difficult to detect the change when two object instances are at the same location. Such augmentation is supported by $Change_{old}^{neg}$. Also, there are small improvements when both the augmentations are used. 


\begin{table}[h]
\caption{Results on applying various augmentations}
\label{tab:results_augmentations}
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Model Name}  & \textbf{Encoder}   & \textbf{Dataset}  & \textbf{F-Score} \\ \hline
\multirow{4}{*}{DeeplabV3+} & \multirow{4}{*}{ResNet - 50} & Original & 0.6684 \\ \cline{3-4} 
 & & \begin{tabular}[c]{@{}c@{}}Instance \\ Augmentation\end{tabular} & 0.6654 \\ \cline{3-4} 
 &  & \begin{tabular}[c]{@{}c@{}}Change \\ Augmentation\end{tabular} & \textbf{0.7057} \\ \cline{3-4} 
 &  & \begin{tabular}[c]{@{}c@{}}Instance + Change \\ Augmentation\end{tabular} & 0.679 \\ \hline
\end{tabular}%
}
\end{table}


\begin{table}[h]
\caption{Results of Change Augmentation on different models}
\label{tab:results_diffmodels}
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Model Name} & \textbf{Encoder}   & \textbf{Dataset}     & \textbf{F-Score} \\ \hline
DeeplabV3+ & \multirow{7}{*}{ResNet - 50} & \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Change \\ Augmentation\end{tabular}} & 0.7057 \\ \cline{1-1} \cline{4-4} 
PSPNet  &  &  & 0.4251 \\ \cline{1-1} \cline{4-4} 
UperNet &  &  & 0.6665 \\ \cline{1-1} \cline{4-4} 
MANet   &  &  & 0.692 \\ \cline{1-1} \cline{4-4} 
LinkNet &  &  & 0.6601 \\ \cline{1-1} \cline{4-4} 
PANet   &  &  & 0.5063 \\ \cline{1-1} \cline{4-4} 
Unet++  &  &  & \textbf{0.7187} \\ \hline
\end{tabular}%
}
\end{table}



\begin{figure}[h]
  \centering
\setkeys{Gin}{width=0.95\linewidth}
  \includegraphics{images/neg2pos_original_pkb9.png}
  \includegraphics{images/neg2pos_both_pkb9.png}
%   \includegraphics{images/NegToPos_Change.png}
%   \includegraphics{images/NegToPos_Both.png}
  \caption{Augmentation of no-change images. Top row: Original image set, Bottom row: Post augmented image set; Left to right: Temporal Image - 1, Temporal Image - 2, Change mask.}
  \label{fig:negtopos}
\end{figure}
\begin{figure}[h]
  \centering
\setkeys{Gin}{width=0.95\linewidth}
  \includegraphics{images/pos2pos_instance_join.png}
  \caption{Instance augmentation of positive images. Top row: Original image set, Bottom row: Post augmented image set; Left to Right:  Temporal Image - 1, Temporal Image - 2, Change mask}
\label{fig:pos2pos_instance}
\end{figure}

\begin{figure}[h]
\centering
\setkeys{Gin}{width=0.95\linewidth}
\includegraphics{images/pos2pos_change_join.png}
\caption{Change mask augmentation of positive images. Top row: Original image set, Bottom row: Post augmented image set; Left to Right:  Temporal Image - 1, Temporal Image - 2, Change mask}
\label{fig:pos2pos_change}  
\end{figure}

\begin{figure}[h]
\centering
\setkeys{Gin}{width=0.95\linewidth}
\includegraphics{images/pos2pos_both_join.png}
\caption{Both instance and change mask augmentation of positive images. Top row: Original image set, Bottom row: Post augmented image set; Left to Right:  Temporal Image - 1, Temporal Image - 2, Change mask}
\label{fig:pos2pos_both}  
\end{figure}




\begin{table}[h]
\caption{F-score compared on different neural network architectures }
\label{tab:results_architectures}
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model Name} & \textbf{Encoder} & \textbf{\begin{tabular}[c]{@{}c@{}}No. of \\ Params \\ in \\ Encoder\end{tabular}} & \textbf{Dataset} & \textbf{F-Score} \\ \hline
\multirow{3}{*}{DeeplabV3+} & ResNet - 18 & 11.174 & \multirow{3}{*}{Original} & 0.6136 \\ \cline{2-3} \cline{5-5} 
 & ResNet - 34 & 21.282 & & 0.6385 \\ \cline{2-3} \cline{5-5} 
 & ResNet - 50 & 23.521 & & \textbf{0.7057} \\ \hline
\end{tabular}%
}
\end{table}

% From Table \ref{tab:results_feature_fusion}, we can observe that concatenating the feature vectors from both the inputs gave the best metric values. The F-score drops for other types of feature fusion, probably due to loss of feature level information, by difference and absolute difference operations. The results in the Table \ref{tab:results_architectures} suggest that with the increasing number of parameters and the model depth the performance metric also improves. 


